From Pixels to Predictions: Spectrogram and Vision Transformer for Better Time Series Forecasting

Time series forecasting plays a crucial role in decision-making across various domains, but it presents significant challenges. Recent studies have explored image-driven approaches using computer vision models to address these challenges, often employing lineplots as the visual representation of time series data. In this paper, we propose a novel approach that uses time-frequency spectrograms as the visual representation of time series data. We introduce the use of a vision transformer for multimodal learning, showcasing the advantages of our approach across diverse datasets from different domains. To evaluate its effectiveness, we compare our method against statistical baselines (EMA and ARIMA), a state-of-the-art deep learning-based approach (DeepAR), other visual representations of time series data (lineplot images), and an ablation study on using only the time series as input. Our experiments demonstrate the benefits of utilizing spectrograms as a visual representation for time series data, along with the advantages of employing a vision transformer for simultaneous learning in both the time and frequency domains.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> nts.tex <==
\subsubsection{NumTS}\label{sec:nts method}
NumTS is a numerical variant of Vision Transformer that received the numerical data as input i.e. only the top price row of an spectrogram image.  NumTS shared the same  architecture with ViT, the only difference between NumTS and ViT was the number of input image patches. NumTS shared the same setup (i.e., mask ratio, loss functions)  as ViT.



==> random_walk.tex <==
\subsubsection{RandomWalk} \label{sec:random_walk}
Random walk without drift was used as a naive numeric forecasting baseline ~\cite{shreve2004stochastic}. This model assumes that the first difference of the time series data is not time-dependent, and follows a Gaussian distribution $\mathcal{N}(0, \sigma)$. Given past time series $\{x_0, \cdots, x_{t-1}, x_t\}$, in order to predict $\{x_{t+1}, \cdots, x_{t+n}\}$, we first estimates $\sigma$ as
\begin{equation*} 
\sigma = \sqrt{\mathop{\mathbb{E}}_{i=1}^{t}[(x_i - x_{i-1})^2]}
\end{equation*}
and the prediction at future time $t+k$ follows
\begin{equation}\label{eq:randomwalk}
    x_{t+k} \sim \mathcal{N}(x_t, \sqrt{k}\sigma)
\end{equation}
which results in a naive numeric forecast that simply extrapolates the last observed value into the future. A growing uncertainty cone can be obtained for the forecast through the equation above.


==> reading.tex <==
\section{Reading}
\subsection{Transformer in NLP}
\begin{itemize}
    \item \textbf{First paper} of Transformer and self-attention Attention mechanism -- \href{https://arxiv.org/abs/1706.03762}{\underline{Attention is all you need}~\cite{vaswani2017attention}}
    \item \textbf{Well explained blog} on transformer and self-attention -- \href{https://jalammar.github.io/illustrated-transformer/}{\underline{blog link}}
    \item \textbf{PyTorch tutorial} on using transformer in NLP -- \href{https://pytorch.org/tutorials/beginner/transformer_tutorial.html}{\underline{tutorial link}}
\end{itemize}

\subsection{Transformer in Computer Vision}
\begin{itemize}
    \item \textbf{First paper} using \textbf{pure} transformer for vision tasks -- \href{https://arxiv.org/abs/2010.11929}{\underline{An Image is worth 16x16 words}~\cite{dosovitskiy2020image}}
    \item \textbf{First paper} to pre-train vision models using the same way large NLP models are trained -- \href{https://arxiv.org/abs/2111.06377}{\underline{MAE: Masked autoencoders are scalable vision learners}~\cite{he2021masked}}
    \textbf{NOTE:} We are going to use the same way to pre-train time series visual models.
    \item \textbf{FAIR PyTorch implementation} of MAE -- \href{https://github.com/facebookresearch/mae}{\underline{github link}}
    \item \textbf{Efficient training} if training takes a long time -- \href{https://arxiv.org/abs/2012.12877}{\underline{Training data-efficient image transformers \& distillation through attention}~\cite{touvron2021training}}
\end{itemize}

\subsection{Time Frequency Spectrum}
\begin{itemize}
    \item \textbf{Tutorial video} on wavelet transform -- \href{https://www.youtube.com/watch?v=kuuUaqAjeoA&ab_channel=AndrewNicoll}{\underline{youtube link}}
    \item \textbf{Medium post} on wavelet transform -- \href{https://towardsdatascience.com/the-wavelet-transform-e9cfa85d7b34}{\underline{medium link}}
    \item \textbf{Scipy functions} for wavelet transform: \href{https://docs.scipy.org/doc/scipy/reference/generated/scipy.signal.cwt.html}{\underline{cwt}}, \href{https://docs.scipy.org/doc/scipy/reference/generated/scipy.signal.morlet2.html}{\underline{morlet2}}
\end{itemize}

==> tft.tex <==
% \subsubsection{TFT} \label{subsec:tft}
% %Give pre-training details 
% We pre-trained and fine-tuned TFT models on classification-based prediction tasks. Unlike masked autoencoder that was pre-trained through self-supervised reconstruction, TFT was not suitable for reconstruction task. Our TFT architecture used 2 layers for the LSTM encoder and decoder with 128-dimensional latent embedding, and a self-attention mechanism with 4 attention heads. We modified the last layer of the TFT model to predict class probabilities by minimizing the cross entropy loss function. For pre-training, We used ranger optimizer with a learning rate of of $1.5\mathrm{e}{-4}$ and a weight decay of 0.02. All other hyperparameters were same as that used in ViTS and NumTS. For fine-tuning, we used the same model hyperparameters as the pre-trained TFT model except the maximum number of epochs was set to 30.
